Three-Body Annihilation of Neutralinos Below Two-Body Thresholds

We calculate the cross section for s-wave neutralino annihilation to three-body final states below the W^+ W^- and t-bar t thresholds. Such three-body channels may dominate the annihilation cross section if the neutralino mass is not too much less than m_t and m_W respectively. Furthermore, because neutrinos produced in these channels are much more energetic than those from the $b\bar{b}$ or tau^+ tau^- channels, they can dominate the energetic-neutrino fluxes from neutralino annihilation in the Sun or Earth far below these thresholds and significantly enhance the neutrino signal in certain regions of the supersymmetric parameter space.

==> prova.tex <==

Prova mandi: 

\vskip5cm
\special{psfile=prova.eps}

\bye

